First Measurements of Beam Backgrounds at SuperKEKB

The high design luminosity of the SuperKEKB electron-positron collider is expected to result in challenging levels of beam-induced backgrounds in the interaction region. Properly simulating and mitigating these backgrounds is critical to the success of the Belle~II experiment. We report on measurements performed with a suite of dedicated beam background detectors, collectively known as BEAST II, during the so-called Phase 1 commissioning run of SuperKEKB in 2016, which involved operation of both the high energy ring (HER) of 7 GeV electrons as well as the low energy ring (LER) of 4 GeV positrons. We describe the BEAST II detector systems, the simulation of beam backgrounds, and the measurements performed. The measurements include standard ones of dose rates versus accelerator conditions, and more novel investigations, such as bunch-by-bunch measurements of injection backgrounds and measurements sensitive to the energy spectrum and angular distribution of fast neutrons. We observe beam-gas, Touschek, beam-dust, and injection backgrounds. We do not observe significant synchrotron radiation, as expected. Measured LER beam-gas backgrounds and Touschek backgrounds in both rings are slightly elevated, on average three times larger than the levels predicted by simulation. HER beam-gas backgrounds are on on average two orders of magnitude larger than predicted. Systematic uncertainties and channel-to-channel variations are large, so that these excesses constitute only 1-2 sigma level effects. Neutron background rates are higher than predicted and should be studied further. We will measure the remaining beam background processes, due to colliding beams, in the imminent commissioning Phase 2. These backgrounds are expected to be the most critical for Belle II, to the point of necessitating replacement of detector components during the Phase 3 (full-luminosity) operation of SuperKEB.

==> crystals_results.tex <==
% file:		crystals_results
% lead author: 	Alex Beaulieu
% timeline:     September 24th


==> daq.tex <==
%     file:		daq.tex
%     author:  	Peter Lewis
%
%     Estimated completion date: End of September

%\textbf{This is all Belle note material. The summary in the paper will probably be 2-3 sentences.}

In this section, we describe the infrastructure and technology we use to unify the disparate parts of BEAST II into one integrated system. This integration occurs at both the hardware and software levels as well as in real-time (``online") and and after completion of runs (``offline"). 

\subsubsection{Shared infrastructure} 
BEAST II uses a decentralized architecture; each subdetector system operates largely independently. However, many resources are shared by all BEAST II systems, particularly networking, shifting, and analysis tools. 

\begin{figure}[htb]
        \centering
        \includegraphics[width=\columnwidth]{BEASTImages/network}
        \caption{A simplified schematic of the general BEAST II networking scheme. From the left, BEAST II hosts live on two private networks, beast\_epics for EPICS traffic, and beast\_daq for everything else. A single machine acts as a Channel Access gateway between beast\_epics and the Belle II slow control network b2\_epics, and as a regular gateway between beast\_daq and the Belle II DAQ network daqnet. The computers used by BEAST II shifters for monitoring of BEAST II and SuperKEKB live on the Belle II networks. A second Channel Access gateway shares select Process Variabless between b2\_epics and the SuperKEKB slow control network skb\_epics (See Sec.~\ref{sec:epics}).}   
        \label{fig:network}
\end{figure}

\subsubsection{Shared infrastructure: networking}
BEAST II subdetector systems share space at the IP, cable paths, and racks, but are only aware of each other as independent hosts on a pair of local Gigabit Ethernet networks. These networks, named beast\_daq and beast\_epics, serve thirteen Linux hosts and a number of Ethernet-capable devices. Figure~\ref{fig:network} shows a simplified schematic of BEAST II networking. 

The beast\_epics network is reserved for BEAST II EPICS traffic, as described in Section~\ref{sec:online_integration}. A gateway between beast\_epics and b2\_epics allows monitoring of live BEAST II data outside the local BEAST II networks. 

The beast\_daq network handles all other network traffic: TCP/IP communication between hosts and a slow control devices, remote SSH access, iSCSI traffic to and from the RAID, and HTTP traffic for local web hosting and connection to cloud services via proxy.  

Two hosts reside outside the local BEAST II networks, on daqnet and b2\_epics (see Figure~\ref{fig:network}). These computers are used by BEAST II shifters to monitor and control BEAST II and compare with SuperKEKB conditions. 

Shared BEAST II resources on the network include a RAID for local data storage, a network switch, and a gateway to KEK internal DAQ and slow control networks (daqnet and b2\_epics, respectively).

\subsubsection{Shared infrastructure: services}
BEAST II users and detector systems rely on a number of shared services. Most of these services are hosted on BEASTmaster, a machine dedicated to this purpose that also serves as the gateway between BEAST II and KEK networks. We describe some of the key services here. 

An archive engine logs BEAST II and selected SuperKEKB PVs in a PostgreSQL database located on the BEAST II RAID. This allows shifters to recall past conditions and provides a backup of detector online products. 

BEASTmaster hosts a Nagios server for systems monitoring, with clients on all hosts. This provides shifters with detailed graphical status reports, automatically emails experts in the event of errors, and logs system performance statistics such as transfer speed, server uptime, and network latency. 

Two ELOG servers are hosted externally at the University of Hawaii, the first dedicated to expert-level BEAST II technical issues and the second to operations and data analysis. This operations ELOG is shared with SuperKEKB and Belle II collaborators and is a key part of sharing BEAST II results. 

A web service hosted on BEASTmaster gives shifters access to HTML documentation for all BEAST II systems. This documentation includes shifting instructions and debugging and troubleshooting guides for each detector.

A network time protocol client and server pair on BEASTmaster and corresponding clients on BEAST II hosts synchronize all BEAST II detectors to the local KEK time servers. This is sufficient for aligning all detectors at the 1~s level required to compare with the 1~Hz SuperKEKB PV values. 

A shared cloud-based spreadsheet contains all beam study run information, maintained by shifters,  with links to the corresponding ELOG entries. The shifters define run numbers with timestamps to direct analysts to the key run periods. 

\subsubsection{Online integration} \label{sec:online_integration}
The primary objective of online integration is to take real-time data and distribute it to BEAST II and SuperKEKB shifters. Conversely, shifters must be able to issue commands to control acquisition devices and set run states. To satisfy both requirements we use the Experimental Physics and Industrial Control System (EPICS), a collection of software tools designed for distributed control systems in large experiments. 

\subsubsection{Online integration: EPICS} \label{sec:epics}
Typical EPICS architecture will consist of a number of Input Output Controllers (IOCs) communicating using client/server or publish/subscribe techniques over a network. An IOC typically serves as the interface between a hardware device and EPICS, and can be thought of as a piece of software that translates between the native language of the device and the native language of EPICS, called Channel Access (CA). CA is used to transmit Process Variables (PVs), which are essentially named pieces of data, usually associated with a hardware device, along with associated metadata like the timestamp of the last update and the units.

In BEAST II, IOCs perform data acquisition, processing, interlocking, and automation. We use EPICS CA libraries inside data acquisition code to skim data in real-time as it is acquired from a device and publish summaries as one or more PVs. In some cases, an independent IOC will read the PV value update and perform further processing of the data and publish its own PVs. Interlock IOCs monitor slow control channels and change device states, for example shutting a high voltage channel off in response to a spike in the monitored current. Finally, state machine IOCs control startup sequences and handle shifter commands.

We use the flexibility of this model of EPICS-based system integration to allow shifters to monitor BEAST II and SuperKEKB conditions in real-time side-by side. In Figure~\ref{fig:network} note the CA gateways between BEAST II and Belle slow control networks (beast\_epics and b2\_epics), and also between the Belle and SuperKEKB slow control networks (b2\_epics and skb\_epics). These gateways transparently broadcast select PVs from one network to the other. In this way, the beast\_epics network is isolated from accelerator PV traffic while allowing the computers used by shifters real-time access to both. In addition, we share select BEAST II PVs with the accelerator network so that SuperKEKB staff can view BEAST II results online.

\subsubsection{Online integration: shifting and user interfacing}
During operation, two BEAST II shifters remain on-site nearly continuously. The first shifter, called the ``Expert", is a BEAST II collaborator with the experience necessary to handle common technical problems. The Expert shifter monitors detector performance and has the authority and training to log into any detector host and restart an IOC, walk to the counting room and reset power supply channels, or notify detector experts in the event of a more serious problem. Finally, the Expert shifter fills a detailed shifting report on ELOG for internal use.

The second shifter, the ``Operator'', is drawn from Belle collaborators, and focuses on comparing BEAST II results with SuperKEKB conditions, communicating with the SuperKEKB group, and producing an ELOG shift report that is shared with external collaborators. 

The user interface for shifters is built in Control System Studio (CSS), a set of tools for interacting with EPICS PVs based on the Eclipse development environment. An operator interface developed in CSS, called an OPI, provides an intuitive graphical layer between the users and EPICS. An OPI typically has plots and gauges to visualize live data, buttons and dials to control devices, tools for accessing archived data, and an interface for alarm handling.

In BEAST II we maintain three OPIs. The first, for BEAST II operator shifters, is focused on comparing SuperKEKB and BEAST II primary data products in real-time and has high-level BEAST II controls. The second, for BEAST II expert shifters, contains highly detailed detector performance data for BEAST II systems only. The third, for BEAST II or SuperKEKB users in the accelerator control room, contains plots similar to what the BEAST II operator shifter sees, but tailored to the most interesting real-time feedback for accelerator operators. 

\subsubsection{Offline integration}
The objective of offline integration is to take data from each subdetector system and combine it into a common data structure. This is essential for comparing subdetector results and analyzing behavior against SuperKEKB conditions. 

Offline integration is not trivial for three primary reasons. First, data from the subdetectors comes in a variety of raw formats. Second, BEAST II has no common trigger and a wide variety of digitization rates and styles. Third, SuperKEKB conditions, such as beam currents, pressures and collimator positions, are not logged by BEAST II but are essential for comprehensive analysis of BEAST II data. 

Our solution to this challenge is to produce a unified set of ROOT {\ntuples} based on 1~s summaries of all relevant BEAST II and SuperKEKB channels. To obtain the SuperKEKB data we download PV values archived in a PostgreSQL database maintained by the accelerator group. In total, the unified BEAST II 
{\ntuples} contain over one hundred branches and nearly one thousand channels. 

\subsubsection{Offline integration: {\ntuple} builder}
To produce standardized {\ntuples} for all BEAST II collaborators, we developed a program that iterates through time at 1~s intervals and summarizes data from all detectors and SuperKEKB for that second. These 1~s summaries are averages, sums, or custom calculations based on entries in the input {\ntuples} that have matching timestamps, rounded down to the nearest second. 

Source data for the {\ntuple} builder includes around ten independent detectors and databases. The {\ntuple} builder is configured through text files that specify which input branches to look for, how to summarize and process them, and what calibrations to apply. This unified approach ensures that all data analysts are using the same calibrations, any plotting script can be shared seamlessly, and analysts have equal access to all BEAST II and SuperKEKB data in a transparent way. The {\ntuples} are provided for each Phase 1 day and for each beam study run. 



==> extrafigs_crystals.tex <==
\subsection{Calibration curves for the crystal calorimeter system} \label{app:Crystal_Cal}

\subsubsection{Dose-dependent calibration}
Figures~\ref{fig:CsI_App_CsITl_Gain_vs_Dose} to \ref{fig:CsI_App_LYSO_Gain_vs_Dose} show the relative gain for the three crystal materials.

%CsI(Tl) channels.
\begin{figure*}[p]
	\begin{subfigure}[a][Channel 0: position F1]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch00-Fit.pdf}
	}
    \end{subfigure}
    %
	\begin{subfigure}[a][Channel 3: position F2]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch03-Fit.pdf}
	}
    \end{subfigure}
    
    \begin{subfigure}[a][Channel 6: position F3]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch06-Fit.pdf}
	}
    \end{subfigure}
    %
    \begin{subfigure}[a][Channel 9: position B1]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch09-Fit.pdf}
	}
    \end{subfigure}
    
    \begin{subfigure}[a][Channel 12: position B2]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch12-Fit.pdf}
	}
    \end{subfigure}
    %
    \begin{subfigure}[a][Channel 15: position B3]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch15-Fit.pdf}
	}
    \end{subfigure}

  \caption{Relative gain of the CsI(Tl) crystal calorimeter channel as a function of total delivered currents}\label{fig:CsI_App_CsITl_Gain_vs_Dose}
\end{figure*}

% Pure CsI Channels
\begin{figure*}[p]
	\begin{subfigure}[a][Channel 1: position F1]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch01-Fit.pdf}
	}
    \end{subfigure}
    %
	\begin{subfigure}[a][Channel 4: position F2]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch04-Fit.pdf}
	}
    \end{subfigure}
    
    \begin{subfigure}[a][Channel 7: position F3]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch07-Fit.pdf}
	}
    \end{subfigure}
    %
    \begin{subfigure}[a][Channel 10: position B1]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch10-Fit.pdf}
	}
    \end{subfigure}
    
    \begin{subfigure}[a][Channel 13: position B2]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch13-Fit.pdf}
	}
    \end{subfigure}
    %
    \begin{subfigure}[a][Channel 16: position B3]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch16-Fit.pdf}
	}
    \end{subfigure}

  \caption[Relative gain of the CsI(pure) crystal calorimeter channel as a function of total delivered currents]{Relative gain of the CsI(pure) crystal calorimeter channel as a function of total delivered currents. The dashed line corresponds to the moment when the high-voltage setting was changed to achieve a factor 2 in gain reduction.}\label{fig:CsI_App_CsIpure_Gain_vs_Dose}
\end{figure*}

% LYSO Channels
\begin{figure*}[p]
	\begin{subfigure}[a][Channel 2: position F1]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch02-Fit.pdf}
	}
    \end{subfigure}
    %
	\begin{subfigure}[a][Channel 5: position F2]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch05-Fit.pdf}
	}
    \end{subfigure}
    
    \begin{subfigure}[a][Channel 8: position F3]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch08-Fit.pdf}
	}
    \end{subfigure}
    %
    \begin{subfigure}[a][Channel 11: position B1]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch11-Fit.pdf}
	}
    \end{subfigure}
    
    \begin{subfigure}[a][Channel 14: position B2]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch14-Fit.pdf}
	}
    \end{subfigure}
    %
    \begin{subfigure}[a][Channel 17: position B3]{
	\includegraphics[width=\columnwidth]{CrystalImages/RelativeGains/Summary_vs_logIint_Ch17-Fit.pdf}
	}
    \end{subfigure}

  \caption{Relative gain of the LYSO crystal calorimeter channel as a function of total delivered currents}\label{fig:CsI_App_LYSO_Gain_vs_Dose}
\end{figure*}

==> extrafigs_diamonds.tex <==
\subsection{Diamonds}
During this phase the diamond sensors and the readout electronics have collected data with full efficiency. The diamond sensors have shown a clear sensitivity to the beam current value, the number of bunches, beam size and the vacuum conditions. The figures from~\ref{fig:currentScanHER_BW_180} to~\ref{fig:currentScanHER_FW_0} show the measured current during the HER current scan while the figures from~\ref{fig:currentScanLER_BW_180} to~\ref{fig:currentScanLER_FW_0} report the results obtained in the LER current scan. Each colour in the plots refer to a different run and each run differs for the number of bunches.
The figures from~\ref{fig:beamGas_BW-180} to~\ref{fig:beamGas_FW-0} show the diamond currents as a function of the product of the HER current value and the average pressure of the residual gas inside the beampipe.
The response of the diamond sensors is proportional to the vacuum level and the beam current and varies with changes in the gas pressure in different regions along the HER beampipe.
The figures from~\ref{fig:touscheck_HER_BW-180} to~\ref{fig:touscheck_HER_FW-0} show the current of diamond sensors as a function of the inverse beam size.
These plots show that the sensor response changes when the HER beam size changes. The increase of the background is due to the inter-beam particles scattering (Touschek effect).
The figures from~\ref{fig:touscheck_LER_BW-180} to~\ref{fig:touscheck_LER_FW-0} show, instead, the response of diamond sensors when the LER beam size is changed.
\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.5]{diamondsImages/currentScanHER_BW_180}
	\caption{The measured current in the BW-180 position as a function of the HER current for different runs. In black the results for run 2001, in red for run 2002, in blu for run 2003 and in magenta for run 2003. Each run differ for the number of bunches, respectively 100\%, 75\%, 50\% and 25\%.}
	\label{fig:currentScanHER_BW_180}
\end{figure}[ht!]
\begin{figure}
	\centering
		\includegraphics[scale=0.5]{diamondsImages/currentScanHER_BW_0}
	\caption{The measured current in the BW-0 position as a function of the HER current for different runs. In black the results for run 2001, in red for run 2002, in blu for run 2003 and in magenta for run 2003. Each run differ for the number of bunches, respectively 100\%, 75\%, 50\% and 25\%.}
	\label{fig:currentScanHER_BW_0}
\end{figure}[ht!]
\begin{figure}
	\centering
		\includegraphics[scale=0.5]{diamondsImages/currentScanHER_FW_180}
	\caption{The measured current in the FW-180 position as a function of the HER current for different runs. In black the results for run 2001, in red for run 2002, in blu for run 2003 and in magenta for run 2003. Each run differ for the number of bunches, respectively 100\%, 75\%, 50\% and 25\%.}
	\label{fig:currentScanHER_FW_180}
\end{figure}

\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.5]{diamondsImages/currentScanHER_FW_0}
	\caption{The measured current in the FW-0 position as a function of the HER current for different runs. In black the results for run 2001, in red for run 2002, in blu for run 2003 and in magenta for run 2003. Each run differ for the number of bunches, respectively 100\%, 75\%, 50\% and 25\%.}
	\label{fig:currentScanHER_FW_0}
\end{figure}

\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.5]{diamondsImages/currentScanLER_BW_180}
	\caption{The measured current in the BW-180 position as a function of the LER current for different runs. In black the results for run 2001, in red for run 2002, in blu for run 2003 and in magenta for run 2003. Each run differ for the number of bunches, respectively 100\%, 75\%, 50\% and 25\%.}
	\label{fig:currentScanLER_BW_180}
\end{figure}

\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.5]{diamondsImages/currentScanLER_BW_0}
	\caption{The measured current in the BW-0 position as a function of the LER current for different runs. In black the results for run 2001, in red for run 2002, in blu for run 2003 and in magenta for run 2003. Each run differ for the number of bunches, respectively 100\%, 75\%, 50\% and 25\%.}
	\label{fig:currentScanLER_BW_0}
\end{figure}

\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.5]{diamondsImages/currentScanLER_FW_180}
	\caption{The measured current in the FW-180 position as a function of the LER current for different runs. In black the results for run 2001, in red for run 2002, in blu for run 2003 and in magenta for run 2003. Each run differ for the number of bunches, respectively 100\%, 75\%, 50\% and 25\%.}
	\label{fig:currentScanLER_FW_180}
\end{figure}

\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.5]{diamondsImages/currentScanLER_FW_0}
	\caption{The measured current in the FW-0 position as a function of the LER current for different runs. In black the results for run 2001, in red for run 2002, in blu for run 2003 and in magenta for run 2003. Each run differ for the number of bunches, respectively 100\%, 75\%, 50\% and 25\%.}
	\label{fig:currentScanLER_FW_0}
\end{figure}



\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.35]{diamondsImages/HERbeamGas_BW_180.png}
	\caption{The measured current in the BW-180 position as a function of the HER current times the average pressure in different regions along the beampipe.}
	\label{fig:beamGas_BW-180}
\end{figure}
\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.35]{diamondsImages/HERbeamGas_BW_0.png}
	\caption{The measured current in the BW-0 position as a function of the HER current times the average pressure in different regions along the beampipe.}
	\label{fig:beamGas_BW-0}
\end{figure}
\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.35]{diamondsImages/HERbeamGas_FW_180.png}
	\caption{The measured current in the FW-180 position as a function of the HER current times the average pressure in different regions along the beampipe.}
	\label{fig:beamGas_FW-180}
\end{figure}
\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.35]{diamondsImages/HERbeamGas_FW_0.png}
	\caption{The measured current in the FW-0 position as a function of the HER current times the average pressure in different regions along the beampipe.}
	\label{fig:beamGas_FW-0}
\end{figure}


\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.45]{diamondsImages/touschek_HER_BW_180.pdf}
	\caption{The measured current in the BW-180 position as a function of the HER inverse beam size.}
	\label{fig:touscheck_HER_BW-180}
\end{figure}
\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.45]{diamondsImages/touschek_HER_BW_0.pdf}
	\caption{The measured current in the BW-0 position as a function of the HER inverse beam size.}
	\label{fig:touscheck_HER_BW-0}
\end{figure}
\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.45]{diamondsImages/touschek_HER_FW_180.pdf}
	\caption{The measured current in the FW-180 position as a function of the HER inverse beam size.}
	\label{fig:touscheck_HER_FW-180}
\end{figure}
\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.45]{diamondsImages/touschek_HER_FW_0.pdf}
	\caption{The measured current in the FW-0 position as a function of the HER inverse beam size.}
	\label{fig:touscheck_HER_FW-0}
\end{figure}

\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.45]{diamondsImages/touschek_LER_BW_180.pdf}
	\caption{The measured current in the BW-180 position as a function of the LER inverse beam size.}
	\label{fig:touscheck_LER_BW-180}
\end{figure}
\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.45]{diamondsImages/touschek_LER_BW_0.pdf}
	\caption{The measured current in the BW-0 position as a function of the LER inverse beam size.}
	\label{fig:touscheck_LER_BW-0}
\end{figure}
\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.45]{diamondsImages/touschek_LER_FW_180.pdf}
	\caption{The measured current in the FW-180 position as a function of the LER inverse beam size.}
	\label{fig:touscheck_LER_FW-180}
\end{figure}
\begin{figure}[ht!]
	\centering
		\includegraphics[scale=0.45]{diamondsImages/touschek_LER_FW_0.pdf}
	\caption{The measured current in the FW-0 position as a function of the LER inverse beam size.}
	\label{fig:touscheck_LER_FW-0}
\end{figure}


==> extrafigs_injectionCry.tex <==
%
\subsection{Injection Background Plots}\label{app:InjCrystal}
We present here the complete set of plots for the eight runs taken during the injection study on May 25, 2016.

\subsubsection{Time Structure}
%In Fig.\,\ref{fig:scaPlotRun3} to \,\ref{fig:scaPlotRun17} 
We show the scalers' hit rate for the LER injection runs \#3, \#6 and \#17. As it is 
apparent from the plots, the overall background for each run appears higher than the reference run \#14 in which the injection was optimised for
maximum efficiency. Run \#17 makes an exception as the background level is very similar to the reference, indicating that the change of the 
. The highest observed change in background 
occurred in run \#3 in which the phase was changed by a large fraction. 
Similarly, %in Fig.\,\ref{fig:scaPlotRun9} to \,\ref{fig:scaPlotRun13} 
we show the scalers' hit rate for the HER injection runs \#9, \#12 and \#13.
As one can see from the difference in the vertical scale, the background levels in the HER are much lower than in the LER also during injection.
Also in this case, it appears that the highest effect is observed in tun \#9 in which the injection phase was changed. 

It is interesting to note, 
%by comparing Fig.\,\ref{fig:scaPlotRun3} and Fig.\,\ref{fig:scaPlotRun9}, 
that the effect of the change of the injection phase, which induces a perturbation in the longitudinal direction, in the HER backgrounds lasts for a longer time than that in 
the LER, which may likely be ascribed to the absence of longitudinal feed-back system in the HER, which is instead present in the LER. 
On the other hand, the time structure of the injection background for the reference run \#10 shows that when the injection phase is optimised the backgrounds
due to injection are very low and they decay in the first 1.5 to 2 ms after injection.

 

\subsubsection{Energy Measurement}
We report the full results of energy fractions in a table. 
%Table\,\ref{tab:HitFracHER} and Table\,\ref{tab:HitFracLER} for the HER and LER, respectively.

%% \begin{table*}[ht]
%%   \centering
%%   \footnotesize{
%%     \begin{tabular}{ lllllll }
%%       \multicolumn{3}{c}{LER}         & RUN \#14 & RUN \#3  & RUN \#6  & RUN \#17  \\  \hline \hline
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       \multirow{9}{*}{\parbox[t]{3cm}{\begin{center}Forward\\Sums\end{center}}} & \multirow{3}{*}{CsI(Tl)} &  $T_{150}$  & ($11.32\pm 0.06$)\%  & ($5.90\pm 0.03$)\%  & ($12.35\pm 0.20$)\%  & ($15.10\pm 0.06$)\% \\ 
%%       & & $T_{bunch}$  & ($1.58\pm 0.02$)\%  & ($1.50\pm 0.02$)\%  & ($1.69\pm 0.07$)\%  & ($2.17\pm 0.02$)\% \\ 
%%       & & $T_{other}$  & ($86.10\pm 0.24$)\%  & ($92.65\pm 0.19$)\%  & ($86.09\pm 0.78$)\%  & ($82.24\pm 0.18$)\% \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%                                \cline{2-7}
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       &\multirow{3}{*}{CsI} & $T_{150}$  & ($31.51\pm 0.21$)\%  & ($42.30\pm 0.29$)\%  & ($36.62\pm 0.35$)\%  & ($50.12\pm 0.30$)\% \\ 
%%       & & $T_{bunch}$  & ($0.12\pm 0.00$)\%  & ($0.11\pm 0.00$)\%  & ($0.10\pm 0.00$)\%  & ($0.37\pm 0.01$)\% \\ 
%%       & & $T_{other}$  & ($66.66\pm 0.32$)\%  & ($51.91\pm 0.22$)\%  & ($61.78\pm 0.46$)\%  & ($47.38\pm 0.24$)\% \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%                                \cline{2-7}
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       &\multirow{3}{*}{LYSO} & $T_{150}$  & ($25.80\pm 0.22$)\%  & ($35.20\pm 0.24$)\%  & ($33.21\pm 0.29$)\%  & ($48.68\pm 0.27$)\% \\ 
%%       & & $T_{bunch}$  & ($1.65\pm 0.02$)\%  & ($3.56\pm 0.03$)\%  & ($2.48\pm 0.03$)\%  & ($3.20\pm 0.03$)\% \\ 
%%       & & $T_{other}$  & ($70.31\pm 0.41$)\%  & ($60.96\pm 0.25$)\%  & ($62.45\pm 0.42$)\%  & ($46.23\pm 0.26$)\% \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       \hline
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       \multirow{9}{*}{\parbox[t]{3cm}{\begin{center}Backward\\Sums\end{center}}} & \multirow{3}{*}{CsI(Tl)} & $T_{150}$  & ($13.59\pm 0.06$)\%  & ($7.79\pm 0.05$)\%  & ($14.76\pm 0.11$)\%  & ($17.71\pm 0.06$)\% \\ 
%%       & & $T_{bunch}$  & ($3.13\pm 0.02$)\%  & ($2.23\pm 0.03$)\%  & ($3.13\pm 0.04$)\%  & ($2.62\pm 0.02$)\% \\ 
%%       & & $T_{other}$  & ($80.58\pm 0.19$)\%  & ($90.08\pm 0.25$)\%  & ($81.24\pm 0.34$)\%  & ($79.65\pm 0.16$)\% \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%                                \cline{2-7}
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       &\multirow{3}{*}{CsI} & $T_{150}$  & ($31.07\pm 0.22$)\%  & ($41.96\pm 0.30$)\%  & ($36.43\pm 0.34$)\%  & ($50.05\pm 0.29$)\% \\ 
%%       & & $T_{bunch}$  & ($0.19\pm 0.00$)\%  & ($0.15\pm 0.00$)\%  & ($0.17\pm 0.00$)\%  & ($0.47\pm 0.02$)\% \\ 
%%       & & $T_{other}$  & ($67.11\pm 0.34$)\%  & ($50.30\pm 0.24$)\%  & ($62.47\pm 0.45$)\%  & ($49.25\pm 0.25$)\% \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%                                \cline{2-7}
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       &\multirow{3}{*}{LYSO} & $T_{150}$  & ($27.47\pm 0.18$)\%  & ($29.76\pm 0.22$)\%  & ($33.13\pm 0.25$)\%  & ($50.27\pm 0.28$)\% \\ 
%%       & & $T_{bunch}$  & ($8.53\pm 0.05$)\%  & ($28.41\pm 0.16$)\%  & ($12.05\pm 0.09$)\%  & ($13.93\pm 0.09$)\% \\ 
%%       & & $T_{other}$  & ($62.51\pm 0.30$)\%  & ($41.00\pm 0.21$)\%  & ($55.03\pm 0.36$)\%  & ($35.51\pm 0.24$)\% \\
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\ \hline\hline
%%     \end{tabular}
%%   }
%%   \caption{Fraction of energy deposited in the three different time regions defined in the text during LER injection. For each crystal type we take the weighted average of the energy measured by the crystals in the 
%% three different positions at $\Phi=0^\circ,~90^\circ,~180^\circ$ separately for the forward and backward positions.}
%%   \label{tab:HitFracLER}
%% \end{table*}

%% \begin{table*}[ht]
%%   \centering
%%   \footnotesize{
%%     \begin{tabular}{ lllllll }
%%       \multicolumn{3}{c}{HER}         & RUN \#10 & RUN \#9  & RUN \#12  & RUN \#13  \\  \hline \hline
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       \multirow{9}{*}{\parbox[t]{3cm}{\begin{center}Forward\\Sums\end{center}}} & \multirow{3}{*}{CsI(Tl)} & $T_{150}$  & ($71.77\pm 0.67$)\%  & ($18.67\pm 0.15$)\%  & ($58.15\pm 0.47$)\%  & ($57.43\pm 0.90$)\% \\ 
%%       & & $T_{bunch}$  & ($14.32\pm 0.14$)\%  & ($9.11\pm 0.06$)\%  & ($8.27\pm 0.09$)\%  & ($9.20\pm 0.20$)\% \\ 
%%       & & $T_{other}$  & ($23.85\pm 0.36$)\%  & ($71.44\pm 0.39$)\%  & ($39.79\pm 0.37$)\%  & ($40.33\pm 0.70$)\% \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%                                \cline{2-7}
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       &\multirow{3}{*}{CsI} & $T_{150}$  & ($81.63\pm 1.33$)\%  & ($12.63\pm 0.26$)\%  & ($68.33\pm 1.83$)\%  & ($69.86\pm 1.03$)\% \\ 
%%       & & $T_{bunch}$  & ($94.13\pm 1.43$)\%  & ($87.42\pm 1.33$)\%  & ($68.67\pm 1.83$)\%  & ($69.67\pm 1.03$)\% \\ 
%%       & & $T_{other}$  & ($4.59\pm 0.11$)\%  & ($9.69\pm 0.19$)\%  & ($26.73\pm 0.65$)\%  & ($25.15\pm 0.27$)\% \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%                                \cline{2-7}
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       &\multirow{3}{*}{LYSO} & $T_{150}$  & -  & ($25.69\pm 0.22$)\%  & ($53.93\pm 1.02$)\%  & ($48.65\pm 1.34$)\% \\ 
%%       & & $T_{bunch}$  & -  & ($71.57\pm 0.46$)\%  & ($50.72\pm 0.99$)\%  & ($45.33\pm 1.30$)\% \\ 
%%       & & $T_{other}$  & -  & ($23.22\pm 0.18$)\%  & ($27.35\pm 0.63$)\%  & ($47.36\pm 1.02$)\% \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       \hline
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       \multirow{9}{*}{\parbox[t]{3cm}{\begin{center}Backward\\Sums\end{center}}} & \multirow{3}{*}{CsI(Tl)} & $T_{150}$  & ($49.65\pm 1.60$)\%  & ($15.91\pm 0.38$)\%  & ($29.13\pm 0.56$)\%  & ($31.05\pm 0.56$)\% \\ 
%%       & & $T_{bunch}$  & ($23.55\pm 0.60$)\%  & ($13.21\pm 0.21$)\%  & ($7.13\pm 0.16$)\%  & ($6.63\pm 0.15$)\% \\ 
%%       & & $T_{other}$  & ($45.03\pm 1.67$)\%  & ($72.45\pm 1.01$)\%  & ($69.42\pm 1.04$)\%  & ($67.38\pm 0.97$)\% \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%                                \cline{2-7}
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       &\multirow{3}{*}{CsI} & $T_{150}$  & ($68.78\pm 2.52$)\%  & ($6.16\pm 0.14$)\%  & ($51.08\pm 1.01$)\%  & ($47.28\pm 0.94$)\% \\ 
%%       & & $T_{bunch}$  & ($32.65\pm 1.24$)\%  & ($54.77\pm 0.56$)\%  & ($12.56\pm 0.30$)\%  & ($11.20\pm 0.26$)\% \\ 
%%       & & $T_{other}$  & ($12.44\pm 0.71$)\%  & ($32.27\pm 0.35$)\%  & ($40.05\pm 0.73$)\%  & ($41.76\pm 0.69$)\% \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%                                \cline{2-7}
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\
%%       &\multirow{3}{*}{LYSO} & $T_{150}$  & -  & ($13.27\pm 0.28$)\%  & ($44.47\pm 1.01$)\%  & - \\ 
%%       & & $T_{bunch}$  & -  & ($0.00\pm 0.70$)\%  & ($0.00\pm 0.94$)\%  & - \\ 
%%       & & $T_{other}$  & -  & ($36.69\pm 0.47$)\%  & ($52.66\pm 0.87$)\%  & - \\ 
%%       \multispan{7}{\rule{0pt}{0.5ex}} \\ \hline\hline
%%     \end{tabular}
%%   }
%%   \caption{Fraction of energy deposited in the three different time regions defined in the text during HER injection. For each crystal type we take the weighted average of the energy measured by the crystals in the 
%% three different positions at $\Phi=0^\circ,~90^\circ,~180^\circ$ separately for the forward and backward positions.}
%%   \label{tab:HitFracHER}
%% \end{table*}


==> extrafigs_pins.tex <==

\subsubsection{Appendix: Calculation of PIN Response to Ionizing Radiation}\label{dose_calculation}

The calculation assumes high energy electrons, as from the $\beta$ sources
we used in our calibration procedures, are minimum
ionizing within the solid silicon of the diode.  We need the
active area of silicon diode ($A = 0.07\,{\rm cm}^{2}$),
the thickness of the silicon diode ($t = 0.02\,{\rm cm}$), the
ionization energy of silicon of 3.6~eV,
minimum ionization for a charged track in silicon of $1.6\,{\rm MeV cm}^{2}/{\rm g}$,
the density of solid silicon ($\rho = 2.33\,{\rm g/cm}^{3}$),
and mass of active area of diode $M = A t \rho = 0.0033\,{\rm gm}$.
A minimum ionizing particle passing through the face of the diode 
deposits $1.6\,{\rm MeV cm}^{2}/{\rm g} \times 2.3\,{\rm g/cm}^{3} \times 0.01\,{\rm cm} = 74\,{\rm keV}$.
This liberates $74\,{\rm keV}/3.6\,{\rm eV} = 20556$~electrons or a charge
of $20556\,{\rm electrons} \times 1.6 \times 10^{-19}\,{\rm C} = 32.89 \times
10^{-16}\,{\rm C}$.  
A $1\,\mu{\rm Ci}$ source produces $3.7 \times 10^{4}$~decays/second
with the fraction hitting the diode $S =  A/(4 \pi d^2)$, where $d$ is the
distance between the diode and an assumed point source.  
For $d = 0.5\,{\rm cm}$, $S = 0.02$, and for $d = 1.0\,{\rm cm}$, $S = 0.0056$.
Thus for $d = 1.0$~cm we expect a current of $32.89 \times 10^{-16}\,{\rm C} 
\times 3.7 \times 10^{4}\,{\rm decays/sec} \times 0.0056 = 0.68\,{\rm pC/sec} = 0.68\,{\rm pA}$. 
According to CREMAT the CR110 preamp has an amplification of 200 mV/nA, but 
bench tests produced 150 mV/nA.  Thus we expect a $1\mu\,{\rm Ci}$ source 
at $1.0$~cm to produce
a voltage output of $0.10$~mV and $0.40$~mV at $0.5$~cm.

A $1\,\mu{\rm Ci}$~Sr-90 source at $1.0$~cm
deposits $74\,{\rm keV} \times 3.7 \times 10^4\,{\rm decays/sec} \times 0.0056/0.0033\,{\rm g}
= 464.63 \times 10^4\,{\rm keV/g-sec} = 0.074\,{\rm mrad/sec}$, and 
similarly for
$0.5$~cm, $0.3$~mrad/sec.  Thus we expect voltage outputs of
$0.1$~mV and $0.4$~mV respectively.  These agree well with the observed
outputs in Table~\ref{table:2} for Sr-90 sources of various 
activities $1.0$~cm from a diode.
Thus the calibration constant for a PIN diode with CR110 preamp is 
$0.75\,\frac{\rm Rad/sec}{\rm V}$.  This calculation is crude with
similar accuracy to the 10\% scatter we observe in the
output of individual diode and preamp combinations.  The overall
accuracy of turning an observed voltage out of an individual
PIN diode into a radiation dose is about 20\%.



\subsubsection{Touschek and vacuum bump study:}\label{pin_appendix}

This section are some plots from Minakshi which should be redundant with the
results section.  They are just here for completeness in the draft
and should be removed on final edit.

Figure~\ref{fig:PIN_LER_diode3} - ~\ref{fig:PIN_LER_diode11} show the phase1 LER Touschek scan result using sensors located at
($\phi$ = 180, z = +15cm), ($\phi$ = 180, z = +3cm), ($\phi$ = 180, z = -11cm).


\begin{figure}[hbt]
 \centering
  \includegraphics[width=3.0in]{PINImages/Phase1_plots/PIN_LER_diode3.pdf}
    \includegraphics[width=3.0in]{PINImages/Phase1_plots/ler_touschek3.pdf}

    \caption{Dose rate (mrad/sec) vs LER inverse beam size ($\mu m^{-1}$) (TOP), and Touschek background fraction vs LER inverse beam size ($\mu m^{-1}$)
    (BOTTOM)  using sensor at ($\phi$,z) = (180, +3cm). }
      \label{fig:PIN_LER_diode3}
\end{figure}


\begin{figure}[hbt]
 \centering
  \includegraphics[width=3.0in]{PINImages/Phase1_plots/PIN_LER_diode15.pdf}
    \includegraphics[width=3.0in]{PINImages/Phase1_plots/ler_touschek15.pdf}

    \caption{Dose rate (mrad/sec) vs LER inverse beam size ($\mu m^{-1}$) (TOP), and Touschek background fraction vs LER inverse beam size ($\mu m^{-1}$)
    (BOTTOM) using sensor at ($\phi$,z) = (180, +15cm). }
      \label{fig:PIN_LER_diode15}
\end{figure}

\begin{figure}[hbt]
 \centering
  \includegraphics[width=3.0in]{PINImages/Phase1_plots/PIN_LER_diode11.pdf}
    \includegraphics[width=3.0in]{PINImages/Phase1_plots/ler_touschek11.pdf}

    \caption{Dose rate (mrad/sec) vs LER inverse beam size ($\mu m^{-1}$) (TOP), and Touschek background fraction vs LER inverse beam size ($\mu m^{-1}$)
    (BOTTOM) using sensor at ($\phi$,z) = (180, -11cm). }
      \label{fig:PIN_LER_diode11}
\end{figure}



Figure~\ref{fig:PIN_HER_diode3} - ~\ref{fig:PIN_HER_diode11} show the phase1 HER Touschek scan result using sensors located at
($\phi$ = 180, z = +15cm), ($\phi$ = 180, z = +3cm), ($\phi$ = 180, z = -11cm).



\begin{figure}[hbt]
 \centering
  \includegraphics[width=3.0in]{PINImages/Phase1_plots/PIN_HER_diode3.pdf}
    \includegraphics[width=3.0in]{PINImages/Phase1_plots/her_touschek3.pdf}

    \caption{Dose rate (mrad/sec) vs HER inverse beam size ($\mu m^{-1}$) (TOP), and Touschek background fraction vs HER inverse beam size ($\mu m^{-1}$)
    (BOTTOM) using sensor at ($\phi$,z) = (180, +3cm). }
      \label{fig:PIN_HER_diode3}
\end{figure}



\begin{figure}[hbt]
 \centering
  \includegraphics[width=3.0in]{PINImages/Phase1_plots/PIN_HER_diode15.pdf}
    \includegraphics[width=3.0in]{PINImages/Phase1_plots/her_touschek15.pdf}

    \caption{Dose rate (mrad/sec) vs HER inverse beam size ($\mu m^{-1}$) (TOP), and Touschek background fraction vs HER inverse beam size ($\mu m^{-1}$)
    (BOTTOM) using sensor at ($\phi$,z) = (180, +15cm). }
      \label{fig:PIN_HER_diode15}
\end{figure}


\begin{figure}[hbt]
 \centering
  \includegraphics[width=3.0in]{PINImages/Phase1_plots/PIN_HER_diode11.pdf}
    \includegraphics[width=3.0in]{PINImages/Phase1_plots/her_touschek11.pdf}

    \caption{Dose rate (mrad/sec) vs HER inverse beam size ($\mu m^{-1}$) (TOP), and Touschek background fraction vs HER inverse beam size ($\mu m^{-1}$)
    (BOTTOM) using sensor at ($\phi$,z) = (180, -11cm). }
      \label{fig:PIN_HER_diode11}
\end{figure}


LER Vacuum bump study using Run 5001-5004:
Four different PIN sensors located at z = -11cm, and $\phi$ = (0, 90, 180, 270) are used to study effect of vacuum bumps around interaction region.
Figure~\ref{fig:PIN_LER_P-bump} shows response of sensors located at $\phi$ = (0, 90, 180, 270) to various vacuum bumps created.
Run 5001, 5002 have large impact on PIN sensors, whereas Run 5003, 5004 have almost no impact. Small $\phi$ dependence for Run 5002 has been observed.

\begin{figure}[hbt]
 \centering
  \includegraphics[width=3.0in]{PINImages/Phase1_plots/5001.pdf}
    \includegraphics[width=3.0in]{PINImages/Phase1_plots/5002.pdf}
     \includegraphics[width=3.0in]{PINImages/Phase1_plots/5003.pdf}
    \includegraphics[width=3.0in]{PINImages/Phase1_plots/5004.pdf}

    \caption{Dose rate (mrad/sec) vs LER current times average pressure for Run 5001 (TOP), Run 5002 (TOP second), Run 5003 (TOP third),
    and Run 5004 (BOTTOM) using sensors at ($\phi$ = 0, z = -11cm), 
  ($\phi$ = 90, z = -11cm), ($\phi$ = 180, z = -11cm), ($\phi$ = 270, z = -11cm).  }
      \label{fig:PIN_LER_P-bump}
\end{figure}


HER Vacuum bump study using Run 6001-6004:
Four different PIN sensors located at z = -11cm, and $\phi$ = (0, 90, 180, 270) are used to study effect of vacuum bumps around interaction region.
Figure~\ref{fig:PIN_HER_P-bump} shows response of sensors located at $\phi$ = (0, 90, 180, 270) to various vacuum bumps created.
Diode at $\phi$ = 180 see little impact to various vacuum bumps created whereas diodes at other $\phi$ locations see no impact.


\begin{figure}[hbt]
 \centering
  \includegraphics[width=3.0in]{PINImages/Phase1_plots/6001.pdf}
    \includegraphics[width=3.0in]{PINImages/Phase1_plots/6002.pdf}
     \includegraphics[width=3.0in]{PINImages/Phase1_plots/6003.pdf}
    \includegraphics[width=3.0in]{PINImages/Phase1_plots/6004.pdf}

    \caption{Dose rate (mrad/sec) vs HER current times average pressure for Run 6001 (TOP), Run 6002 (TOP second), Run 6003 (TOP third),
    and Run 6004 (BOTTOM) using sensors at ($\phi$ = 0, z = -11cm), 
  ($\phi$ = 90, z = -11cm), ($\phi$ = 180, z = -11cm), ($\phi$ = 270, z = -11cm). }
      \label{fig:PIN_HER_P-bump}
\end{figure}



==> extrafigs_tpc.tex <==
\subsection{TPCs}
\subsubsection{TPC Detector Performance Plots}

\begin{figure}[hbt]
\begin{center}
\includegraphics[width=\columnwidth]{TPCimages/tpc3_deltat.eps}
\includegraphics[width=\columnwidth]{TPCimages/tpc4_deltat.eps}
\caption[single column]{$\Delta t$ distribution of sequential neutron events, in seconds for channels 3 (top) and 4 (bottom).  We note that there is no significant source of detector downtime at the 1 second level.}
\label{fig_tpc_deltat}
\end{center}
\end{figure}

%\begin{figure}[hbt]
%\includegraphics[width=8cm]{TPCimages/tpc3_deltat.eps}
%\caption[single column]{$\delta t$ distribution of sequential neutron events, in seconds for channel 3.  We note that there is no significant source of detector downtime at the 1 second level.}
%\label{fig_tpc3_deltat}
%\end{figure}


%\begin{figure}[hbt]
%\includegraphics[width=8cm]{TPCimages/tpc4_deltat.eps}
%\caption[single column]{$\delta t$ distribution of sequential neutron events, in seconds for channel 4.  We note that there is no significant source of detector downtime at the 1 second level.}
%\label{fig_tpc4_deltat}
%\end{figure}


==> mechanical_survey.tex <==
%     file:&&mechanical_survey.tex
%     authors:  &Alexandre Beaulieu
%     timeline:         September 10th
%
%     contents:





 
 \subsection{Position measurements}\label{sec:geomPos}
The positions of each sub-detector was measured using a combination of Bosch GLM50 laser ranging device, measuring tape and plumb bob. The detector positions recorded correspond to the origin of the volume defined in the Geant4 description of the detector: generally but not necessarily the center-of-mass of the sensitive volume.  Due to the many reference changes needed to report each position with respect to the nominal interaction point located inside the beampipe, the uncertainty of each coordinate is estimated to be $\pm20\text{~mm}$. 

Tables~\ref{tab:TPC-Position} to \ref{tab:PIN-Position} present the result of the position survey for each detector. The index associated with each read-out channel is also reported to enable cross-links between these tables and the recorded and simulated data.

% Switch to symbol footnotes for tables to avoid confusion with exponents
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}

%
\begin{table}[ht!]
\caption{Positions of the micro Time Projection Chambers}\label{tab:TPC-Position}
\centering
\begin{tabular}{lcrrr}
\toprule
Name & Index\footnotemark[1] & \multicolumn{3}{c}{Position (mm)} \\
                       & & $x$ & $y$ & $z$ \\
\midrule
TPC1\footnotemark[2] & N/A &   N/A &  N/A & N/A\\
TPC2\footnotemark[2] & N/A &   N/A &  N/A & N/A\\
TPC3 & N/A & -477 &   62 & 342\\
TPC4 & N/A &  -66 & -450 & 388\\
\bottomrule
\end{tabular}
\parbox{\columnwidth}{\footnotemark[1]{\footnotesize The TPC data are not recorded as an array of channels in the recorded and simulated {\ntuples}}}
\parbox{\columnwidth}{\footnotemark[2]{\footnotesize TPC1 and TPC2 were inactive for the duration of Phase 1}}
\end{table}
%

%
\begin{table}[ht!]
\caption{Positions of the crystal calorimeter units}\label{tab:CSI-Position}
\centering
\begin{tabular}{lcrrr}
\toprule
Name & Indices\footnotemark[1] & \multicolumn{3}{c}{Position (mm)} \\
           & & $x$ & $y$ & $z$ \\
\midrule
CRY-F1 & $\{ 0, 1, 2\}$ &  498 &  -5 &  2158\\ 
CRY-F2 & $\{ 3, 4, 5\}$ &  -26 & 522 &  2147\\ 
CRY-F3 & $\{ 6, 7, 8\}$ & -533 &  -4 &  2157\\ 
CRY-B1 & $\{ 9,10,11\}$ &  587 & -12 & -1234\\
CRY-B2 & $\{12,13,14\}$ &  -27 & 618 & -1241\\
CRY-B3 & $\{15,16,17\}$ & -618 &  -8 & -1250\\
\bottomrule
\end{tabular}
\parbox{\columnwidth}{\footnotemark[1]{\footnotesize Indices are given as \{CsI(Tl), CsI(pure) and LYSO\} for channels in each calorimeter unit}}
\end{table}
%

\begin{table}[ht!]
\caption{Positions of the $^3$He neutron detectors}\label{tab:He3-Position}
\centering
\begin{tabular}{lcrrr}
\toprule
Name & Index & \multicolumn{3}{c}{Position (mm)} \\
                       & & $x$ & $y$ & $z$ \\
\midrule
He3-0   & 0 &  464 &   99 & 325\\
He3-90  & 1 & -135 &  493 & 340\\
He3-180 & 2 & -504 & -109 & 338\\
He3-270 & 3 &  105 & -477 & 384\\
\bottomrule
\end{tabular}
\end{table}
%
\begin{table}[ht!]
\caption{Positions of the beam-abort diamond sensors}\label{tab:Diamonds-Position}
\centering
\begin{tabular}{lcrrr}
\toprule
Name & Index & \multicolumn{3}{c}{Position (mm)} \\
           & & $x$ & $y$ & $z$ \\
\midrule
DC-3B & 0 &  49 &  3 &  109\\
DM-4  & 1 &  50 &  6 &  -97\\
DM-7B & 2 & -48 &  4 &  109\\
DM-5  & 3 & -46 &  1 &  -97\\
\bottomrule
\end{tabular}
\end{table}
%

\begin{table}[ht!]
\caption{Positions of the CLAWS sensors}\label{tab:CLAWS-Position}
\centering
\begin{tabular}{lcrrr}
\toprule
Name & Index & \multicolumn{3}{c}{Position (mm)} \\
           & & $x$ & $y$ & $z$ \\
\midrule
CLAWS-FWD-1 & 0 &  172 & 63&  2053 \\
CLAWS-FWD-2 & 1 &  278 & 66&  2050 \\
CLAWS-FWD-3 & 2 &  387 & 67&  2055 \\
CLAWS-FWD-4 & 3 &  676 & 67&  2057 \\
CLAWS-BWD-1 & 4 & -144 & 62& -1127 \\
CLAWS-BWD-2 & 5 & -254 & 61& -1132 \\
CLAWS-BWD-3 & 6 & -360 & 61& -1134 \\
CLAWS-BWD-4 & 7 & -467 & 63& -1137 \\
\bottomrule
\end{tabular}
\end{table}
%

\begin{table}[ht!]
\caption{Positions of the BGO crystals}\label{tab:BGO-Position}
\centering
\begin{tabular}{lcrrr}
\toprule
Name & Index & \multicolumn{3}{c}{Position (mm)} \\
           & & $x$ & $y$ & $z$ \\
\midrule
BGO-1 & 3 & 119 &  119 &  396  \\ 
BGO-2 & 5 & -82 &  122 & -294  \\ 
BGO-3 & 4 & 130 &  103 & -275  \\ 
BGO-4 & 1 & -86 &  108 &  396  \\ 
BGO-5 & 2 & -90 & -196 &  396  \\ 
BGO-6 & 0 &  77 & -177 &  396  \\ 
BGO-7 & 6 & -81 & -145 & -294  \\ 
BGO-8 & 7 & 104 & -153 & -293  \\ 
\bottomrule
\end{tabular}
\end{table}

\begin{table}[ht!]
\caption{Positions of the PIN diode sensors}\label{tab:PIN-Position}
\centering
\begin{tabular}{lcrrr}
\toprule
Name & Indices\footnotemark[1] & \multicolumn{3}{c}{Position (mm)} \\
           & & $x$ & $y$ & $z$ \\
\midrule
PIN-1-0   & $\{ 35,~39\}$ & 104 &  12 & -1265 \\
PIN-1-90  & $\{ 24,~28\}$ &  -7 &  56 & -1265 \\
PIN-1-180 & $\{ 25,~29\}$ &-108 &  -2 & -1265 \\
PIN-1-270 & $\{ 34,~38\}$ &   3 & -58 & -1265 \\
PIN-2-0   & $\{ 27,~31\}$ &  81 &   9 &  -710 \\
PIN-2-90  & $\{ 32,~36\}$ &   2 &  58 &  -710 \\
PIN-2-180 & $\{ 26,~30\}$ & -86 &   9 &  -710 \\
PIN-2-270 & $\{ 33,~37\}$ &   2 & -56 &  -710 \\
PIN-3-0   & $\{ 19,~22\}$ &  52 &  -7 &  -119 \\
PIN-3-90  & $\{  2,~ 3\}$ &   8 &  49 &  -120 \\
PIN-3-180 & $\{  4,~ 5\}$ & -49 &  -7 &  -121 \\
PIN-3-270 & $\{ 18,~23\}$ &  -5 & -49 &  -120 \\
PIN-4-0   & $\{ 16,~17\}$ &  55 &   1 &    31 \\
PIN-4-90  & $\{  8, ~9\}$ &   9 &  49 &    30 \\
PIN-4-180 & $\{  0,~ 1\}$ & -49 &  -3 &    30 \\
PIN-4-270 & $\{ 20,~21\}$ &   2 & -49 &    30 \\
PIN-5-0   & $\{ 14,~15\}$ &  51 &   0 &   143 \\
PIN-5-90  & $\{  7,~10\}$ &   5 &  49 &   145 \\
PIN-5-180 & $\{  6,~11\}$ & -51 &  -4 &   144 \\
PIN-5-270 & $\{ 12,~13\}$ &  14 & -49 &   144 \\
PIN-6-0   & $\{ 48,~52\}$ &  86 &  -3 &   710 \\
PIN-6-90  & $\{ 47,~40\}$ &  -9 &  58 &   710 \\
PIN-6-180 & $\{ 49,~53\}$ & -83 &  -5 &   710 \\
PIN-6-270 & $\{ 46,~41\}$ &  -8 & -53 &   710 \\
PIN-7-0   & $\{ 45,~42\}$ & 109 &  -7 &  1344 \\
PIN-7-90  & $\{ 50,~54\}$ & -25 &  58 &  1344 \\
PIN-7-180 & $\{ 51,~55\}$ &-137 & -12 &  1344 \\
PIN-7-270 & $\{ 44,~43\}$ & -15 & -54 &  1344 \\
PIN-TPC-1 & $\{ 59,~58\}$ & 475 &  40 &   325 \\
PIN-TPC-2 & $\{ 56,~57\}$ & -61 & 507 &   358 \\
PIN-TPC-3 & $\{ 61,~63\}$ &-506 & -40 &   335 \\
PIN-TPC-4 & $\{ 60,~62\}$ &  32 &-494 &   324 \\
\bottomrule
\end{tabular}
\parbox{\columnwidth}{\footnotemark[1]{\footnotesize Indices are given as \{Au coated, no coating\} for channels in each PIN diode unit}}
\end{table}





% Switch back to arabic footnote marks so as not to affect the rest of the document
\renewcommand*{\thefootnote}{\arabic{footnote}}


==> simulation_detectors.tex <==
%     file:		simulation_detectors.tex
%     authors:  	Igal Jaegle
%
\label{simulation_detectors}

The geometry and materials of the BEAST II sensors, support structures, beampipes, and cave are implemented in {\GEANT} \cite{g4} embedded in 
basf2. For the particles' interaction with matter and their transport, we use the {\GEANT} $QGSP\_BERT\_HP$ hadronic model with the data-driven 
high precision neutron package (HP), for neutrons below 20 MeV down to thermal energies, except for charged particle transport in the gaseous TPCs. Since in one second-equivalent 
simulation, a few hundreds neutrons are crossing the TPCs resulting at most to one elastic recoils from a neutron, all neutrons crossing the micro-TPC sensitive volumes in one 
second are re-launched 3600 times to mimic one hour-equivalent simulation. Furthermore to calculate properly the ionization energy in the TPC gas, all charged particles 
interacting with the gas are re-launched using a modified {\GEANT} package based on the standard electromagnetic physics builder and a screened Coulomb collisions model coupled with the 
Linhard theoretical curve for the energy loss in the gas of ions (and protons), and the {\GEANT} PAI model for charged particles lighter than a nucleon.

The modeling of the electromagnetic calorimeters and counters (Crystals and BGO) response is done by folding the energy resolution, $\sigma$, into the energy deposited, $E_{dep}^{G4}$, calculated
 by the {\GEANT} physics model, as follows:
\begin{equation}
E_{dep} = E_{dep}^{G4} + \frac{\sigma}{\sqrt{E_{dep}^{G4}}} 
\end{equation}
and by taking into account the energy threshold and the energy dynamic range induced by the electronic readout. For the Crystals the 
energy threshold did change during the course of the measurement, therefore the hit rate, Figure~\ref{fig:CSI_HitRate_thres} ,and dose, Figure~\ref{fig:CSI_Dose_thres}, as a function of 
the energy threshold are also modeled for each channel, ring, and background type by a polynomial of order six. Because, the energy distribution of the electromagnetic showers 
induced by the beams is different for each background type, ring and $(r,\phi,z)$.

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{SimulationImages/CSI_HitRate_thres.pdf}
\caption{Hit rate as a function of the energy threshold for each 18 channels of the Crystals system. The distributions were fitted by a polynomial of order six.}
\label{fig:CSI_HitRate_thres}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{SimulationImages/CSI_Dose_thres.pdf}
\caption{Dose as function of the energy threshold for each 18 channels of the Crystals system. The distributions were fitted by a polynomial of order six}
\label{fig:CSI_Dose_thres}
\end{figure}


For the ionization radiation sensors, PIN and Diamond, and the gaseous detectors, $^{3}$He and TPC, the {\GEANT} energy deposited is converted into charged, 
$N_{e^-}$, if the energy deposited is above the work function $W$, as followed:
\begin{equation}
N_{e^-}^{mean} =  E_{dep}^{G4} / W
\end{equation}
where $N_{e^-}^{mean}$ is the mean charged, Then, the resolution, $\sigma$ , is deduced from the Fano Factor, $F$, and the mean charged as:
\begin{equation}
\sigma = \sqrt{F \times N_{e^-}^{mean} }
\end{equation}
Finally, the charge, $N_{e^-}$, is calculated according to a Gaussian distribution with mean, $N_{e^-}^{mean}$, and width, $\sigma$.
For the ionization radiation sensors, we convert back into energy, $E_{dep}$, the charge could deposit using:
\begin{equation}
E_{dep} = N_{e^-} \times W, 
\end{equation} 

The table~\cite{tab:gas} below gives the Work Function and Fano Factor used for PIN and Diamond, 1 atm $He:CO_2:70:30$, and 3 atm $^3He:CO_2:95:5$.

\begin{table}
  \caption{Work function and Fano factor for the radiation sensors (PIN amd Diamond) and gaseous detectors ($^{3}$He tubes and TPC)}
  \label{tab:gas}
  \begin{tabular}{|c|c|c|}
    \toprule
    Sensor&Work function [eV]&Fano factor\\
    \midrule
    PIN & 3.64 & 0.13\\
    Diamond & 13.25 & 0.382\\
    $He:CO_2:70:30$ & 35.075 & 0.19\\
    $^3He:CO_2:95:5$ & 24.6 & 0.22 \\
    \bottomrule
  \end{tabular}
\end{table}

In addition to these steps, for the gaseous detector, the charges' drift to the amplification stage (GEMs and wire for the TPC and $^{3}$He~tubes, respectively) and plane
readout (for the TPC) is simulated by a fast Monte Carlo simulation using the gas properties calculated by MAGBOLTZ \cite{magboltz}. The charge readout by the plane or wire is then
 digitized by reproducing the digital output of the electronic readout. Figures~\ref{fig:NeutronEvent, fig:ProtonEvent, fig:ElectronEvent} show simulation of a reconstructed
alpha recoil produced  by a neutron elastically scattering off the $^4$He-gas, a proton track produced by neutron elastically scattering off plastic material surrounding the
sensitive gas volume,  and an electron emitted by the shower produced by the beam hitting the beampipes, respectively. For each TPC, we use the gas parameters
corresponding to the pressure measured.  For each TPC, we use the gas parameters corresponding to the pressure measured, voltages applied, estimated GEMs gain,
and estimated gas absorption by the analysis of the two internal calibration sources.

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{SimulationImages/NeutronEvent.png}
\caption{A typical alpha recoil produced by a neutron elastically scattering off the $^4$He-gas. Left: 3D plot. Right: 2D plot}
\label{fig:NeutronEvent}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{SimulationImages/ProtonEvent.png}
\caption{A typical proton track produced by a neutron elastically scattering off plastic material surrounding the sensitive gas volume. Left: 3D plot. Right: 2D plot}
\label{fig:NeutronEvent}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{SimulationImages/ElectronEvent.png}
\caption{An electrom emitted by the shower produced by the beam hitting the beampipes. Left: 3D plot. Right: 2D plot}
\label{fig:NeutronEvent}
\end{figure}


For the plastic scintillators, QCSS and CLAWS, the light saturation or Birk's law is used to calculate the (attenuated) energy deposited in \GEANT. The attenuated energy deposited is 
converted into Minimum Ionization Particle (MIP) which is then converted into Photon Electron (PE) per time window slice, the detailed numbers are in Table~\cite{tab:sci}. 

%table column heading split to better fit with document column width.
\begin{table}
  \caption{Conversion factors from \GEANT deposited energy to Photoelectrons (PE) for CLAWS and QCSS.}
  \label{tab:sci}
  \begin{tabular}{|c|c|c|c|c|}
    \hline
    Sensor & kev/MIP & MIP/PE & Threshold [PE] & Time window\\ 
           &         &        &                & [ns]\\
    \hline
    CLAWS & 467.11 & 12 to 16 & 1 & 8\\
    QCSS &  1628.20 & 15 & 0.5 & -\\
    \hline
  \end{tabular}
\end{table}

The conversion energy to MIP is determined by simulation, Figures~\cite{fig:QCSS_MIP} and~\cite{fig:CLAWS_MIP}. The {\GEANT} energy deposited in CLAWS/QCSS by one GeV muon beam, 
perpendicular to the horinzonthal plan, is fitted by a Landau function to determine the most probable value of the Landau density which is the MIP.

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{SimulationImages/QCSS_MIP.pdf}
\caption{\GEANT energy deposited in QCSS by one GeV muon beam}
\label{fig:QCSS_MIP}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{SimulationImages/CLAWS_MIP.pdf}
\caption{\GEANT energy deposited in CLAWS by one GeV muon beam.}
\label{fig:CLAWS_MIP}
\end{figure}

The modeling of the detector response is validated by comparing the simulation to laboratory measurements done with calibration sources if available. For the PIN diodes, we simulate the measurements done at Wayne State University with 3 $^{60}Co$ sources of different activities. Figure \cite{fig:PIN_validation} shows that the simulation is in good agreement with the data.

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{SimulationImages/PIN_validation.pdf}
\caption{Output versus source activity for the PIN system.}
\label{fig:PIN_validation}
\end{figure}

The modeling of the Diamond response is validated by comparing the energy deposited simulated by Fluka and {\GEANT} by 1 MeV normal incident electron beam, see Figure~\cite{fig:DIA_validation}. Fluka and {\GEANT} are in good 
agreement.

\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{SimulationImages/DIA_FLUKA_G4.pdf}
\caption{Energy deposited by 1 MeV normal incident electron beam. Simulated by Fluka (blue point) and {\GEANT} (red square).}
\label{fig:DIA_validation}
\end{figure}



==> simulation_handoff.tex <==
% File: simulation_readers.tex
% Lead author: Igal Jaegle

The Phase 1 beam loss positions, momenta, and rates in the IR are calculated with SAD and the synchroton radiation software as described in Section~\ref{simulation_generation}. In addition, the SAD loss positions are given at the exit of the slice and do not correspond to the exact loss position which is occurring upstream. Therefore we transform into the {\GEANT} coordinate system and correct the SAD coordinates in order to be equal to or smaller than the aperture size set in SAD by using the (exact) momentum provided by SAD. This can be achieved iteratively by moving upstream by a fixed step of $ds$ = 10~$\mu$m, which we find to be the optimal step size.
The number of (primary) particles launched by {\GEANT} at each loss position corresponds to the calculated loss rate attached to the particle lost scaled by a time equivalent to the running accelerator beam time, which is typically 1~s for one {\GEANT} simulation and each background type and ring. The SAD loss rate has non-negligible statistical uncertainty which depends on the number of particles launched at the injection point and the number of SAD simulations done and introduces a systematic error on the simulated {\GEANT} sensor rates and doses. 





==> thermal_neutrons_analysis.tex <==
\subsection{Thermal neutrons: analysis}
\label{thermal_neutrons_analysis}

\subsubsection{Introduction}

Presented here is an alternative simulation weighting scheme and analysis which was performed only on the \heT tube data. The experimental data used here is the same as in Section \ref{subsec:touschek_approach}, as shown in Table \ref{tab:touschek_runs}. It was discovered that there was some unknown scaling factor on the pressure measured by the pressure gauges on the beampipes. Additionally, while there was information on the gas mixture in the LER beampipe (see Section \ref{sec:Zeff}), there was no information on the HER beampipe's gas mixture, as there were no RGAs there. The goal of this analysis is to quantify this pressure scaling factor and, for the HER, account for the gas mixture in the beampipe. This is done by forcing the ratio of the Touschek rate to the beam-gas rate in simulation to be the same as in the experimental data. This is presented as a complementary analysis to that presented in Section \ref{subsec:touschek_approach}.



%This analysis determines the \heT tube averaged ratio of the Touschek and beam-gas contributions to the rate from the experimental data, then scales the beam-gas component of the simulation to produce the same ratio. This ratio contains the pressure scaling factor and (for the HER) information about the gas mixture.







\subsubsection{Scaling of Simulation}
\label{sec:samsim2}

\begin{figure}[htb]
	\includegraphics[scale=0.6]{thermalAnalysisImages/SKEKb_key}
	\caption{SuperKEKB ring showing `D' sections.}
	\label{fig:SKB2}
\end{figure}

The beam-gas and Touschek components of the background are simulated separately for fixed beam parameters, as seen in Section~\ref{simulation_weighting}. Each component is then scaled to match the measured beam parameters by re-weighting the events produced with SAD and GEANT by the scale value at that moment in time. The same simulated events are reused for all beam settings.

The scaled beam-gas rate predicted by simulated is given by:
\begin{equation}
	{R_{\mathrm{BG}}^{\mathrm{Scaled}} = \sum _{i=1}^{12}(R^{\mathrm{Brems}}_i+R^{\mathrm{Coulomb}}_i)\cdot\frac{P_{\mathrm{scale}}(I\cdot P_i\cdot Z_{\mathrm{e}~i}^{2})_{\mathrm{experiment}}} {(I\cdot P\cdot Z^{2})_{\mathrm{sim}}}}
\label{eq:simScale2}
\end{equation}
where $R^{\mathrm{Brems}}_{i}$ and $R^{\mathrm{Coulomb}}_{i}$ are the components of the inelastic and elastic beam-gas simulated rates produced in each $^3$He tube from interaction at each `D' section of the HER and LER rings (see Fig. \ref{fig:SKB2}), $P_{i}$ is the pressure in each `D' section, and $Z_{\mathrm{e}~i}$ is the effective atomic number of the gas in each section (see Eq.~\ref{eqn:Ze}), if available. If $Z_{\mathrm{e}~i}$ is not available in a `D' section, 2.7 is used for the LER (since this was near the mean value of $Z$ during the experiment, see Section.~\ref{sec:TousExp}), and 1 is used in the HER.  $P_{\mathrm{scale}}$ is a scale factor on the overall pressure to account for the fact that the measurement made by the uncalibrated pressure gauges is proportional to the actual pressure. This scale factor will be discussed further in Section.~\ref{sec:TousExp}.

The scaled Touschek component of the simulation is given by:
\begin{equation}
	{R_{\mathrm{Tous}}^{\mathrm{Scaled}} = R_{\mathrm{Tous}}\cdot\frac{(I^{2}/N_{\mathrm{Bunch}}\cdot\sigma_{y})_{\mathrm{experiment}} }{(I^{2}/N_{\mathrm{Bunch}}\cdot\sigma_{y})_{\mathrm{sim}}}}
\end{equation}
where $R_{\mathrm{Tous}}$ is the Touschek simulated rate, $\sigma_{y}$ is the vertical beam size, and $N_{\mathrm{Bunch}}$ is the number of filled bunches in the ring.

These scaled components are combined to obtain the predicted rate of thermal neutrons in each $^3$He tube,
\begin{equation}
	{R_{\mathrm{Sim}} = \varepsilon_{^3\mathrm{He}}\left(R_{\mathrm{BG}}^{\mathrm{Scaled}}+R_{\mathrm{Tous}}^{\mathrm{Scaled}}\right)}
\end{equation}
where $\varepsilon_{^3\mathrm{He}}$ is the efficiency of each \heT tube, as shown in Table \ref{tab:he3Calib}. %The scaling parameters for the beam-gas and Touschek backgrounds are consistent with the discussion in Chapter \ref{chap:beamBack}.



%In order to verify that these scale factors are appropriate, a SAD simulation was done at different beam parameters than listed in Table \ref{tab:SimBeam}. This was compared to a scaled version of the nominal simulation, which showed this scaling approach to be appropriate.





\subsubsection{Analysis}
\label{sec:TousExp2}

	In order to separate the beam-gas and Touschek component of the \heT tube rate during the beam size scans, both the measured rate and the simulated rate is fit to this function:
\begin{equation}
	{R_{^{3}\mathrm{He tube}} = c_{\mathrm{gas}}\cdot P\cdot I\cdot Z_{\mathrm{e}}^{2}+c_{\mathrm{T}}\cdot \frac{I^{2}}{N_{\mathrm{Bunch}}\cdot\sigma_{y}}}
	\label{eqn:TousFit2}
\end{equation}
where $P$ is the pressure in the beampipe, $I$ is the beam current, $Z_{\mathrm{e}}$ is the effective atomic number of the beampipe gas, $\sigma_{y}$ is the vertical size of the beam, and $c_{\mathrm{gas}}$ and $c_{\mathrm{T}}$ are the fit parameters. Fig.~\ref{fig:tousZef2} demonstrating how $Z_{\mathrm{e}}$ changes during the beam size runs, showing the importance of including it in the fit. For the LER, the value of $Z_{\mathrm{e}}$ measured at D02 is used since it is closest to the IR. This technique is described in detail in Section.~\ref{sec:RGAMethodology}. The HER has no RGA, and therefore it is not possible to determine the value of $Z_{\mathrm{e}}$, so a value of 1 is assumed. The $P_{\mathrm{scale}}$ factor used in the simulation scaling (see Section.~\ref{sec:samsim2}) is 1.


For each subrun, the averages of the $^3$He rate, $P\cdot I\cdot Z_{\mathrm{e}}^{2}$, and $\frac{I^{2}}{N_{\mathrm{Bunch}}\cdot\sigma_{y}}$ are calculated. These are the input parameters of the fit in Eq.~\ref{eqn:TousFit2}.


\begin{figure}
	\centering
		\includegraphics[width=\columnwidth]{thermalAnalysisImages/Zeff}
	\caption[$Z_{\mathrm{e}}$ during LER beam size runs]{$Z_{\mathrm{e}}$ during LER beam size runs examined in this analysis. Data were recorded on May 17, 2016.}	
	\label{fig:tousZef2}
\end{figure}

The results of this fit for experiment and simulation for LER and HER (in $^3$He tube number 0 (0$^{\circ}$)) are shown in Figs.~\ref{fig:LERTous102} and~\ref{fig:HERTous102} respectively. The experiment is divided into three runs, each with five subruns. The runs occurred at different beam currents, and the subruns each had different vertical beam sizes. In these figures, the black points are the average measured \heT tube rates in each subrun. The Touschek component, in yellow, is given by:
\begin{equation}
	R_{\mathrm{T}} = c_{\mathrm{T}}\cdot \frac{I^{2}}{N_{\mathrm{Bunch}}\cdot\sigma_{y}}
\end{equation}
and the beam-gas component, in blue, is given by:
\begin{equation}
	R_{\mathrm{gas}} = c_{\mathrm{gas}}\cdot P\cdot I\cdot Z_{\mathrm{e}}^{2}
\end{equation}
The error bars shown are the standard deviation of the \heT tube rate for that subrun. The pressure in the beampipe is changing over the course of the experiments and is included in the fit through the $c_{\mathrm{gas}}\cdot P\cdot I\cdot Z_{\mathrm{e}}^{2}$ component, but for simplicity the pressure changes during the subruns are not shown in the figures. The values produced by the fit can be found in Table~\ref{tab:FitPars2}, and $\chi^2$ and number of degrees of freedom (ndf) are in Table~\ref{tab:ChiNDF}. Note that only statistical errors and fit parameters uncertainties are included in the $\chi^2$ calculation. If the systematic errors are included, $\chi^2$ becomes significantly smaller. Note that $\chi^2$ for the fits to simulation are not equal to 1. This is because the fiting function (Eq. \ref{eqn:TousFit2}) is different than the scaling function (Eq. \ref{eq:simScale2}).



\begin{sidewaystable}
    \centering
    \begin{tabular}{cc|cc|cc|cccc}
\toprule
	&		&		 \multicolumn{2}{c}{Experiment}								&	 \multicolumn{2}{c}{Simulation – Initial Scaling} 							&	 \multicolumn{2}{c}{Simulation – Corrected Scaling}    							\\	
	&	 	&		 c$_{gas}$				&	 c$_{T}$			&	 c$_{gas}$			&	 c$_{T}$ 			&	 c$_{gas}$			&	 c$_{T}$ 			\\	
	&	Channel 	&		  [$Hz/(mA\cdot Pa)$]				&	 [$Hz\cdot\mu m/mA^{2}$]			&	 [$Hz/(mA\cdot Pa)$]			&	 [$Hz\cdot\mu m/mA^{2}$]  			&	  [$Hz/(mA\cdot Pa)$]			&	 [$Hz\cdot\mu m/mA^{2}$]  			\\	
\midrule
HER	&	0 (0$^\circ$)	&	(	2.409	$\pm$	0.047	)$\times10^{5}$	&	0.229	$\pm$	0.039	&	198	$\pm$	13	&	0.11483	$\pm$	0.00010	&	79133	$\pm$	848	&	0.089	$\pm$	0.007	\\	
	&	1 (90$^\circ$)	&	(	1.097	$\pm$	0.036	)$\times10^{5}$	&	0.120	$\pm$	0.030	&	170	$\pm$	18	&	0.16646	$\pm$	0.00015	&	66805	$\pm$	742	&	0.144	$\pm$	0.006	\\	
	&	2 (180$^\circ$)	&	(	1.752	$\pm$	0.033	)$\times10^{5}$	&	0.212	$\pm$	0.027	&	93	$\pm$	4	&	0.03634	$\pm$	0.00003	&	37608	$\pm$	415	&	0.026	$\pm$	0.003	\\	
	&	3 (270$^\circ$)	&	(	2.413	$\pm$	0.035	)$\times10^{5}$	&	0.224	$\pm$	0.029	&	151	$\pm$	9	&	0.08302	$\pm$	0.00008	&	60616	$\pm$	651	&	0.064	$\pm$	0.005	\\	\hline
LER	&	0 (0$^\circ$)	&		6170	$\pm$	475		&	17.0	$\pm$	0.6	&	323.5	$\pm$	0.9	&	4.408	$\pm$	0.0011	&	1881	$\pm$	3	&	4.428	$\pm$	0.004	\\	
	&	1 (90$^\circ$)	&		3294	$\pm$	213		&	8.3	$\pm$	0.3	&	328.0	$\pm$	1.0	&	5.309	$\pm$	0.0013	&	1905	$\pm$	3	&	5.330	$\pm$	0.004	\\	
	&	2 (180$^\circ$)	&		5584	$\pm$	308		&	13.7	$\pm$	0.4	&	187.0	$\pm$	0.6	&	2.832	$\pm$	0.0007	&	1087	$\pm$	2	&	2.844	$\pm$	0.002	\\	
	&	3 (270$^\circ$)	&		7677	$\pm$	448		&	18.8	$\pm$	0.6	&	255.0	$\pm$	0.7	&	3.630	$\pm$	0.0009	&	1482	$\pm$	3	&	3.646	$\pm$	0.003	\\	
\bottomrule


    \end{tabular}
    \caption[Parameters associated with fits for each \heT tube channel]{Results of fitting for the Touschek and beam-gas components, $c_{\mathrm{gas}}$ and $C_T$, of the thermal neutron rate in each $^3$He tube. $\chi^2$ and ndf can be found in Table~\ref{tab:ChiNDF}. Initial scaling is with $P_{\mathrm{scale}}$=1, and corrected scaling is with $P_{\mathrm{scale}}$ as defined shown in Table~\ref{tab:meanPScale}.}
    \label{tab:FitPars2}
\end{sidewaystable}


\begin{sidewaystable}
    \centering
    \begin{tabular}{ccccc}
\toprule
	&		&		&	Simulation	&	Simulation	\\	
	&		&	 Experiment	&	Initial Scaling	&	Corrected Scaling	\\	
	&	Channel	&	$\chi^2$	&	$\chi^2$	&	$\chi^2$	\\	
\midrule
HER	&	0 (0$^\circ$)	&	7.19	&	2.40	&	15.17	\\	
	&	1 (90$^\circ$)	&	9.99	&	2.32	&	15.87	\\	
	&	2 (180$^\circ$)	&	6.05	&	2.56	&	15.93	\\	
	&	3 (270$^\circ$)	&	7.28	&	2.42	&	15.44	\\	
\midrule
LER	&	0 (0$^\circ$)	&	109.6	&	1.33	&	24.51	\\	
	&	1 (90$^\circ$)	&	75.0	&	1.06	&	18.93	\\	
	&	2 (180$^\circ$)	&	89.7	&	1.12	&	20.68	\\	
	&	3 (270$^\circ$)	&	88.7	&	1.23	&	22.86	\\	
\bottomrule


    \end{tabular}
    \caption[$\chi^2$ for fits for each \heT tube channel]{$\chi^2$ for fits for each \heT tube channel. Note that only the statistical errors and fit parameter uncertainties are included in the calculation of $\chi^2$. ndf = 12 for all fits.}
    \label{tab:ChiNDF2}
\end{sidewaystable}



\begin{figure}
	\centering
		\includegraphics[width=\columnwidth]{thermalAnalysisImages/LERTousFirstPass_0}
	\caption[Result of fitting Eq.~\ref{eqn:TousFit2} to the measured (top) and simulated (bottom) thermal neutron rates for Touschek experiments in \heT tubes, LER, channel 0]{Result of fitting Eq.~\ref{eqn:TousFit2} to the measured (top) and simulated (bottom) thermal neutron rates for  Touschek experiments in \heT tubes, LER, channel 0. Yellow (color available online) is the Touschek component, blue is the beam-gas component, and black is the rate measured in \heT tube channel 0. Error bars are the standard deviation of the mean of the rate in that bin and are too small to be seen on this scale.}	
	\label{fig:LERTous10}
\end{figure}




\begin{figure}
	\centering
		\includegraphics[width=\columnwidth]{thermalAnalysisImages/HERTousFirstPass_0}
		\caption{Result of fitting Eq.~\ref{eqn:TousFit2} to the measured (top) and simulated (bottom) thermal neutron rates for Touschek experiments in \heT tubes, HER, channel 0. Yellow (color available online) is the Touschek component, blue is the beam-gas component, and black is the rate measured in \heT tube channel 0. Error bars are the standard deviation of the mean of the rate in that bin and are too small to be seen on this scale.}	
	\label{fig:HERTous10}
\end{figure}






As evident from Fig.~\ref{fig:HERTous102}, the simulation greatly underestimates the beam-gas component in the HER, and to a lesser extent in the LER. This is due to two factors: $Z_{\mathrm{e}}$ is not known in the HER, and $P_{\mathrm{scale}}$ is not known in either beam. Using a value of 1 for these parameters does not give the correct beam-gas component. To compensate, the ratio of the beam-gas fit parameter, $c_{gas}$, to the Touschek fit parameter, $c_{T}$, for experiment is used to estimate a value for $P_{\mathrm{scale}}Z_{\mathrm{e}}^{2}$ (or simply $P_{\mathrm{scale}}$ for the LER, since $Z$ is known) that is used in the weighting of each channel in the simulation:
\begin{equation}
	{P_{\mathrm{scale}}Z_{\mathrm{e}}^{2} = \frac{(c_{\mathrm{gas}}/c_{\mathrm{T}})_{\mathrm{experiment}}}{(c_{\mathrm{gas}}/c_{\mathrm{T}})_{\mathrm{sim}}}}
\label{eqn:Pscale1}
\end{equation}
The motivation for this is that all the parameters of the Touschek component of the fit are relatively well known, while the pressure and $Z_{\mathrm{e}}$ in the beam-gas component are not. The beam-gas to Touschek ratio in the experiment is used to determine $P_{\mathrm{scale}}Z_{\mathrm{e}}^{2}$ to be used in the simulation weighting. Note that this does not constrain the overall total prediction of the background from the simulation or the absolute individual contributions.

\begin{figure}
	\centering
	\subfigure{
		\begin{overpic}[width=\columnwidth]{thermalAnalysisImages/LERPScale}
		\end{overpic}
		\label{fig:LERPScale2}
	}
	\subfigure{
		\begin{overpic}[width=\columnwidth]{thermalAnalysisImages/HERPScale}
		\end{overpic}
		\label{fig:HERPScale2}
	}
	\caption{LER and HER $P_{\mathrm{scale}}$ and $P_{\mathrm{scale}}Z_{\mathrm{e}}^{2}$. The vertical line is the weighted mean.}	
	\label{fig:PScaleZsq2}
\end{figure}

\begin{table}[htb]
	\centering
	\begin{tabular}{ ccc }
\toprule
				&	Weighted mean	&	Uncertainty	\\	
\midrule
$P_{\mathrm{scale}}$ (LER)			&	5.84	&  0.20	\\		
$P_{\mathrm{scale}}Z_{\mathrm{e}}^{2}$ (HER)	&	417	&  37		\\	
\bottomrule

	\end{tabular}
	\caption{Weighted mean of $P_{\mathrm{scale}}$}
	\label{tab:meanPScale2}
\end{table}


The values for $P_{\mathrm{scale}}Z_{\mathrm{e}}^{2}$ can be found in Fig.~\ref{fig:PScaleZsq2}. Note that the values are significantly different between LER and HER. This is because the $Z_{\mathrm{e}}$ is known for the LER, but not the HER. 

The simulation was then re-weighted by the weighted mean of $P_{\mathrm{scale}}$ (see Table~\ref{tab:meanPScale2}), and the experiment and simulation were again fit to Eq.~\ref{eqn:TousFit2}. The results of the fit for LER and HER (in channel 0 (0$^{\circ}$)) are shown in Figs.~\ref{fig:LERTous202} and~\ref{fig:HERTous202} respectively. The values of the fit parameters can be found in Table~\ref{tab:FitPars2}.



\begin{figure}
	\centering
		\includegraphics[width=\columnwidth]{thermalAnalysisImages/LERTousSecondPass_0}
	
	\caption[Result of fitting Eq.~\ref{eqn:TousFit} to the measured (top) and simulated (bottom) thermal neutron rates for Touschek experiments after simulation is weighted by $P_{\mathrm{scale}}$, LER, channel 0]{Result of fitting Eq.~\ref{eqn:TousFit} to the measured (top) and simulated (bottom) thermal neutron rates for  Touschek experiments after simulation is weighted by $P_{\mathrm{scale}}$, LER, channel 0. Yellow (color available online) is the Touschek component, blue is the beam-gas component, and black is the rate measured in \heT tube channel 0. Error bars are the standard deviation of the mean of the rate in that bin and are too small to be seen on this scale.}	
	\label{fig:LERTous202}
\end{figure}



\begin{figure}
	\centering
		\includegraphics[width=\columnwidth]{thermalAnalysisImages/HERTousSecondPass_0}
	
	\caption[Result of fitting Eq.~\ref{eqn:TousFit} to the measured (top) and simulated (bottom) thermal neutron rates for Touschek experiments after simulation is weighted by $P_{\mathrm{scale}}Z_{\mathrm{e}}^{2}$, HER, channel 0]{Result of fitting Eq.~\ref{eqn:TousFit} to the measured (top) and simulated (bottom) thermal neutron rates for  Touschek experiments after simulation is weighted by $P_{\mathrm{scale}}Z_{\mathrm{e}}^{2}$ , HER, channel 0. Yellow (color available online) is the Touschek component, blue is the beam-gas component, and black is the rate measured in \heT tube channel 0. Error bars are the standard deviation of the mean of the rate in that bin and are too small to be seen on this scale.}	
	\label{fig:HERTous202}
\end{figure}


%--------------rewrite----------------------






	In order to verify the overall accuracy of the simulation, a ratio of the experiment to simulation is defined:
\begin{subequations}
\begin{align}
		{(D/S) = \frac{\Sigma R_{\mathrm{data}}} {\Sigma R_{\mathrm{sim}}}} 
\end{align}
\end{subequations}

The more accurate the simulation, the closer these ratios will be to 1. These ratios can also be used to scale the simulation to better match the experiment. The values of these ratios can be found in Table~\ref{tab:dataSimRatio2}. %Note that the table omits the uncertainty on the ratio. This is discussed in detail in Section.~\ref{sec:Systematics}.

\begin{table}[htb]
	\centering
	\begin{tabular}{ ccc }
\toprule
Channel	&	$(D/S)_{\mathrm{HER}}$	&	$(D/S)_{\mathrm{LER}}$	\\	
\midrule
0 (0$^\circ$)	&	2.99	&	3.68	\\		
1 (90$^\circ$)	&	1.49	&	1.61	\\		
2 (180$^\circ$)	&	4.93	&	4.92	\\		
3 (270$^\circ$)	&	3.94	&	5.16	\\	
\bottomrule


	\end{tabular}
	\caption[Ratio of experiment to simulation for beam-gas and Touschek parameters]{Ratio of experiment to simulation for beam-gas and Touschek parameters.}
	\label{tab:dataSimRatio2}
\end{table}

\paragraph{Estimating the Uncertainty on $(D/S)$}

\begin{table}[htb]
	\centering
	\begin{tabular}{ ccc }
\toprule
	&	LER	&	HER	\\	
\midrule
I (mA)	&	0.03	&	0.03	\\		
$\sigma_{y}$	&	1.37\%	&	3.71\%	\\		
$P_{\mathrm{scale}}Z_{\mathrm{e}}$	&	0.20	&	36.6	\\	
\bottomrule

	\end{tabular}
	\caption[Uncertanties on current, beam size, and $P_{\mathrm{scale}}Z_{\mathrm{e}}^{2}$]{Uncertanties on current, beam size, and $P_{\mathrm{scale}}Z_{\mathrm{e}}^{2}$~\cite{samsThesis}.}
	\label{tab:paramUncert2}
\end{table}


To estimate the systematic uncertainty from beam current, beam size, $P_{\mathrm{scale}}Z_{\mathrm{e}}^{2}$, and \heT tube efficiency, the simulation was re-weighted with each quantity separately adjusted to +1$\sigma$ and -1$\sigma$ values. The full analysis was then redone. For example:
\begin{subequations}
\begin{align}
		{I\rightarrow I+0.03\mathrm{~mA}} \\
		{I\rightarrow I-0.03\mathrm{~mA}}
\end{align}
\end{subequations}
and similarly for $\sigma_{y}$ and $P_{\mathrm{scale}}$Z$^{2}$ (for more details, see~\cite{samsThesis}). The uncertanity on each parameter can be found in Table~\ref{tab:paramUncert2}. The analysis described in Section.~\ref{sec:TousExp2} was repeated to get new values of (D/S). These were used to calculate the systematic error for each quantity:
\begin{subequations}
\begin{align}
	{\sigma_{(D/S)_{+}}^{I} = (D/S)|_{I=I+0.03\mathrm{~mA}} - (D/S)|_{\mathrm{nominal}}} \\
	{\sigma_{(D/S)_{-}}^{I} = (D/S)|_{\mathrm{nominal}} - (D/S)|_{I=I-0.03\mathrm{~mA}} }
\end{align}
\end{subequations}

\begin{table}[htb]
	\centering
	\begin{tabular}{ cccccccc }
\toprule
	&	I	&	\multicolumn{2}{c}{$\sigma_y$}			&	\multicolumn{2}{c}{$P_{\mathrm{scale}}$}			&	\multicolumn{2}{c}{$\epsilon_{^3He}$}			\\	
HER	&$\sigma$		&	$\sigma_{+}$	&	$\sigma_{-}$	&	$\sigma_{+}$	&	$\sigma_{-}$	&	$\sigma_{+}$	&	$\sigma_{-}$	\\
\midrule
0	&	0	&	0.016	&	0.017	&	0.24	&	0.21	&	0.24	&	0.23	\\	
1	&	0	&	0.012	&	0.013	&	0.11	&	0.09	&	0.12	&	0.11	\\	
2	&	0	&	0.018	&	0.020	&	0.42	&	0.36	&	0.40	&	0.38	\\	
3	&	0	&	0.020	&	0.021	&	0.32	&	0.28	&	0.32	&	0.30	\\	
\midrule
LER	&		&		&		&		&		&		&		\\	
0	&	0	&	0.035	&	0.035	&	0.039	&	0.039	&	0.30	&	0.28	\\	
1	&	0	&	0.016	&	0.016	&	0.015	&	0.015	&	0.13	&	0.12	\\	
2	&	0	&	0.048	&	0.049	&	0.049	&	0.048	&	0.40	&	0.38	\\	
3	&	0	&	0.050	&	0.050	&	0.054	&	0.052	&	0.42	&	0.39	\\	
\bottomrule




	\end{tabular}
	\caption{Systematic uncertanties on (D/S).}
	\label{tab:RatioWithErrors2}
\end{table}





Table~\ref{tab:RatioWithErrors2} contains the numerical values of the systematic uncertainty from each source. 



%	The total uncertainty shown in Table~\ref{tab:RatioWithErrors} is the sum in quadrature of the uncertainty from each separate component. The major contributor to the uncertainty on the experiment/simulation ratio is the uncertainty due to the tubes being at different $\phi$ locations. This uncertainty is associated with the difference between the measured and simulated neutron flux at each different \heT tube. A large uncertainty here shows that the simulation is incorrectly predicting the $\phi$ dependency of the neutron flux.


%------------------------------------------------------------------------------------------------












==> thermal_neutrons_results.tex <==
\subsection{Thermal neutron results}
\label{thermal_neutrons_results}


\begin{figure}
	\centering
		\includegraphics[width=\columnwidth]{thermalAnalysisImages/RatioPlot}
	\caption{LER and HER data simulation ratios vs versus azimuthal angle  of detector.}	
	\label{fig:RatioWithErrors2}
\end{figure}



The average ratio of data to simulation with uncertainties in the is 3.33$\pm$0.11 in the LER data and is 3.84$^{+0.59}_{-0.51}$ for the HER. Fig.~\ref{fig:RatioWithErrors2} shows the (D/S) for each \heT tube. There is good agreement for the \heT tubes at 0$^o$, 90$^o$, and 180$^o$ but some difference for the tube at 270$^o$. The disagreement in (D/S) between the four \heT tubes shows that the simulation is not accurately predicting the $\phi$ distribution of the thermal neutrons.



==> usop.tex <==
\subsection{Crystals temperature and relative humidity monitoring system}\label{sec:usop}

\begin{figure}
\centering
\includegraphics[width=8.5cm]{img/usop.png}
\caption{Aggregation scheme of the uSOP system for the forward boxes. The same scheme applies to backward boxes.}
\label{fig:uSOP_scheme}
\end{figure}

The scintillation of crystals depends on temperature, moreover they are known to be hygroscopic and an excess of absorbed humidity may reduce the light yield (LY) permanently. Expected variations in LY at room temperature can be of a few percent per degree Celsius for the CsI(Tl) crystals. Therefore, we arranged a dedicated system, named Service Oriented Platform based on uP (uSOP), for monitoring temperature (T) of each crystal and the relative humidity (RH) in the boxes hosting them. 
The uSOP system is a single-board computer custom designed for monitoring T and RH of crystals in the Belle2 electromagnetic calorimeter (ECL). 
Among its peripherals uSOP includes 16 general purpose digital IOs, a 4-channel 12-bit ADC and several field buses ports (2 UARTs, 1 JTAG port, 2 I2Cs and 2 SPIs). uSOP is designed to be expanded by means of peripheral boards connected to one of the field bus port, which are transformer-coupled. This in turns permits to reduce ground loops and to protect the uSOP main board from electrostatic discharges (ESD).
In its setup for BEAST, each uSOP system is connected via SPI bus to two 24-bit ADC peripheral boards and it monitors three boxes (Fig.~\ref{fig:uSOP_scheme}). For each box, the humidity is measured by means of a Vaisala HMP60 relative humidity probe \cite{Vaisala:probe}, while the temperature is measured by means of three Semitec AT-2 thermistors \cite{AT:thermistor}, one per crystal. The temperature and humidity sensors are the same model adopted in the Belle2 ECL.
The sensors are routed on a patch printed circuit board ("cable adapter") installed on the side of the box. From there a 40m 16-pin shielded cable routes the signals to the counting room, where the uSOP crate is installed.
The thermistors are read according to the so-called three-wire scheme, in such a way to cancel out the effect of the the cable parasitic resistance. Moreover, the specific acquisition mode supported by the ADC (Linear LTC2983 \cite{Linear:ADC}) interfaced to uSOP, permits to remove even effects related to parasitic thermocouples (e.g. metal-metal junctions in contacts). 

The system is capable to measure the temperature with an uncertainty of $\pm$0.3\degree C and relative humidity with an uncertainty of $\pm$3\%.  
The acquired data are transferred by uSOP via a network connection, according to the EPICS protocol and they can be charted by EPICS-compliant tools such as CS Studio (Fig.~\ref{fig:uSOP_trends}).

\begin{figure}
\centering
\includegraphics[width=8.5cm]{img/usop_trends.png}
\caption{Trends of temperature and relative humidity PVs provided by the uSOP system.}
\label{fig:uSOP_trends}
\end{figure}

Two Input Output Controllers (IOCs) run on the uSOP main-board and they provide process variables (PVs) for the temperature and dew point for each crystal and the relative humidity of the box. The PVs are logged onto files by a server machine and at the same time charted on cloud websites (such as Beebotte) in order to be monitored easily from anywhere.  It would be also possible, though not implemented yet, to provide information about the frost point and the total amount of water in the box volume.

